QuAILoRA: Quantization-Aware Initialization for LoRA

QLoRA reduces the memory-cost of fine-tuning a large language model (LLM) with LoRA by quantizing the base LLM. However, quantization introduces quantization errors that negatively impact model performance after fine-tuning. In this paper we introduce QuAILoRA, a quantization-aware initialization for LoRA that mitigates this negative impact by decreasing quantization errors at initialization. Our method spends a small amount of computational overhead to compute this quantization-aware initialization, without increasing the memory-cost of fine-tuning. We evaluate our method on several causal language modeling and downstream evaluation tasks using several different model sizes and families. We observe that almost all LLMs fined-tuned with QuAILoRA achieve better validation perplexity. When evaluated on downstream tasks, we find that QuAILoRA yields improvements proportional to the negative effect of quantization error. On average, applying QuAILoRA to 4-bit QLoRA models yields 75% of the validation perplexity decrease and 86% of the downstream task accuracy increase as doubling the quantization precision to 8-bit, without increasing GPU memory utilization during fine-tuning.

==> fig/downstream_tasks.tex <==
\begin{table*}[!t]
\centering
\begin{subtable}{\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Method & Model & Arc-C & Arc-E & BoolQ & HS & OBQA & PIQA & WinoG & avg. \\
\hline
QLoRA & 7b 4-bit & 42.9\tiny$\pm$1.4 & 73.3\tiny$\pm$0.9 & 72.5\tiny$\pm$0.8 & 55.7\tiny$\pm$0.5 & \textbf{35.0}\tiny$\pm$2.1 & 77.9\tiny$\pm$1.0 & 69.1\tiny$\pm$1.3 & 60.9 \\
Ours & 7b 4-bit & \textbf{44.8}\tiny$\pm${1.5} & \textbf{74.4}\tiny$\pm${0.9} & \textbf{74.0}\tiny$\pm${0.8} & \textbf{55.8}\tiny$\pm$0.5 & 34.6\tiny$\pm$2.1 & \textbf{78.7}\tiny$\pm$1.0 & \textbf{70.9}\tiny$\pm${1.3} & \bf 61.9 \\
\hline
QLoRA & 7b 8-bit & 44.4\tiny$\pm$1.5 & \textbf{73.8}\tiny$\pm$0.9 & \textbf{75.7}\tiny$\pm$0.8 & 55.9\tiny$\pm$0.5 & 35.8\tiny$\pm$2.1 & 78.7\tiny$\pm$1.0 & \textbf{71.1}\tiny$\pm$1.3 & 62.2 \\
Ours & 7b 8-bit & \textbf{44.7}\tiny$\pm$1.5 & \textbf{73.8}\tiny$\pm$0.9 & 75.1\tiny$\pm$0.8 & \textbf{56.5}\tiny$\pm${0.5} & \textbf{37.4}\tiny$\pm$2.2 & \textbf{78.9}\tiny$\pm$1.0 & 71.0\tiny$\pm$1.3 & \textbf{62.5} \\
\hline
QLoRA & 13b 4-bit & 46.3\tiny$\pm$1.5 & 75.0\tiny$\pm$0.9 & 82.0\tiny$\pm$0.7 & \textbf{59.3}\tiny$\pm${0.5} & \textbf{36.4}\tiny$\pm$2.2 & \textbf{78.8}\tiny$\pm$1.0 & \textbf{73.2}\tiny$\pm$1.2 & \textbf{64.4} \\
Ours & 13b 4-bit & \textbf{46.9}\tiny$\pm$1.5 & \textbf{75.2}\tiny$\pm$0.9 & \textbf{82.4}\tiny$\pm$0.7 & 58.7\tiny$\pm$0.5 & 35.8\tiny$\pm$2.1 & 78.7\tiny$\pm$1.0 & 72.5\tiny$\pm$1.3 & 64.3 \\
\hline
QLoRA & 13b 8-bit & \textbf{47.5}\tiny$\pm$1.5 & \textbf{75.3}\tiny$\pm$0.9 & \textbf{82.3}\tiny$\pm$0.7 & \textbf{59.0}\tiny$\pm$0.5 & \textbf{35.4}\tiny$\pm$2.1 & \textbf{79.2}\tiny$\pm$0.9 & \textbf{73.6}\tiny$\pm$1.2 & \textbf{64.6} \\
Ours & 13b 8-bit & 46.8\tiny$\pm$1.5 & 75.2\tiny$\pm$0.9 & \textbf{82.3}\tiny$\pm$0.7 & \textbf{59.0}\tiny$\pm$0.5 & 34.6\tiny$\pm$2.1 & 78.9\tiny$\pm$1.0 & 73.2\tiny$\pm$1.2 & 64.3 \\
\hline
QLoRA & 30b 4-bit & 51.5\tiny$\pm$1.5 & \textbf{79.3}\tiny$\pm$0.8 & \textbf{86.5}\tiny$\pm$0.6 & \textbf{61.5}\tiny$\pm${0.5} & 38.2\tiny$\pm$2.2 & 81.3\tiny$\pm$0.9 & \textbf{74.7}\tiny$\pm$1.2 & \textbf{67.6} \\
Ours & 30b 4-bit & \textbf{52.6}\tiny$\pm$1.5 & \textbf{79.3}\tiny$\pm$0.8 & 86.1\tiny$\pm$0.6 & 61.3\tiny$\pm${0.5} & \textbf{38.4}\tiny$\pm$2.2 & \textbf{81.4}\tiny$\pm$0.9 & 74.0\tiny$\pm$1.2 & \textbf{67.6} \\
\hline
QLoRA & 30b 8-bit & 53.2\tiny$\pm$1.5 & \textbf{80.3}\tiny$\pm$0.8 & 85.8\tiny$\pm$0.6 & \textbf{62.3}\tiny$\pm$0.5 & \textbf{38.4}\tiny$\pm$2.2 & \textbf{81.4}\tiny$\pm$0.9 & \textbf{74.7}\tiny$\pm$1.2 & 68.0 \\
Ours & 30b 8-bit & \textbf{53.8}\tiny$\pm$1.5 & 80.1\tiny$\pm$0.8 & \textbf{86.5}\tiny$\pm$0.6 & 62.2\tiny$\pm$0.5 & 38.2\tiny$\pm$2.12& 81.3\tiny$\pm$0.9 & \textbf{74.7}\tiny$\pm$1.2 & \textbf{68.1} \\
\hline
\end{tabular}
\caption{Downstream task performance for LLaMA models fine-tuned on Alpaca}
\end{subtable}

\begin{subtable}{\textwidth}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Method & Model & Arc-C & Arc-E & BoolQ & HS & OBQA & PIQA & WinoG & avg. \\
\hline
QLoRA & 7b 4-bit & 41.6\tiny$\pm$1.4 & 75.0\tiny$\pm$0.9 & 80.0\tiny$\pm$0.7 & 57.4\tiny$\pm$0.5 & \textbf{35.0}\tiny$\pm$2.1 &	78.3\tiny$\pm$1.0 & 69.2\tiny$\pm$1.3 & 62.3 \\
Ours & 7b 4-bit & \textbf{42.7}\tiny$\pm$1.4 & \textbf{75.5}\tiny$\pm$0.9 & \textbf{80.6}\tiny$\pm$0.7 & \textbf{57.8}\tiny$\pm$0.5 & 34.4\tiny$\pm$2.1 & \textbf{78.6}\tiny$\pm$1.0 & \textbf{71.0}\tiny$\pm${1.3} & \textbf{62.9}  \\
\hline
QLoRA & 7b 8-bit & \textbf{43.1}\tiny$\pm$1.4 & 75.1\tiny$\pm$0.9 & 80.8\tiny$\pm$0.7 & 58.3\tiny$\pm$0.5 & \textbf{36.6}\tiny$\pm$2.2 & \textbf{78.5}\tiny$\pm$1.0 & 69.2\tiny$\pm$1.3 & \textbf{63.1} \\
Ours & 7b 8-bit & 42.6\tiny$\pm$1.4 & \textbf{75.2}\tiny$\pm$0.9 & \textbf{81.3}\tiny$\pm$0.7 & \textbf{58.4}\tiny$\pm$0.5 & 35.6\tiny$\pm$2.1 & \textbf{78.5}\tiny$\pm$1.0 & \textbf{70.1}\tiny$\pm$1.3 & \textbf{63.1} \\
\hline
QLoRA & 13b 4-bit & \textbf{49.3}\tiny$\pm$1.5 & 78.6\tiny$\pm$0.8 & \textbf{83.8}\tiny$\pm$0.6 & 60.0\tiny$\pm$0.5 & 37.0\tiny$\pm$2.2 & \textbf{79.2}\tiny$\pm$0.9 & 72.8\tiny$\pm$1.2 & \textbf{65.8} \\
Ours & 13b 4-bit & \textbf{49.3}\tiny$\pm$1.5 & \textbf{79.0}\tiny$\pm$0.8 & 83.2\tiny$\pm$0.7 & \textbf{60.1}\tiny$\pm$0.5 & \textbf{37.2}\tiny$\pm$2.2 & 78.3\tiny$\pm$1.0 & \textbf{72.9}\tiny$\pm$1.2 & 65.7 \\
\hline
QLoRA & 13b 8-bit & 49.1\tiny$\pm$1.5 & 78.6\tiny$\pm$0.8 & \textbf{83.8}\tiny$\pm$0.6 & 60.4\tiny$\pm$0.5 & \textbf{37.4}\tiny$\pm$2.2 & 78.9\tiny$\pm$1.0 & \textbf{72.9}\tiny$\pm$1.2 & \textbf{65.9} \\
Ours & 13b 8-bit & \textbf{49.5}\tiny$\pm$1.5 & \textbf{78.9}\tiny$\pm$0.8 & 83.4\tiny$\pm$0.7 & \textbf{60.5}\tiny$\pm$0.5 & 36.2\tiny$\pm$2.2 & \textbf{79.4}\tiny$\pm$0.9 & 72.8\tiny$\pm$1.3 & 65.8 \\
\hline
QLoRA & 30b 4-bit & \textbf{56.0}\tiny$\pm$1.5 & \textbf{82.4}\tiny$\pm$0.8 & \textbf{87.2}\tiny$\pm$0.6 & \textbf{63.5}\tiny$\pm$0.5 & \textbf{38.4}\tiny$\pm$2.2 & \textbf{81.5}\tiny$\pm$0.9 & 75.2\tiny$\pm$1.2 & \textbf{69.2} \\
Ours & 30b 4-bit & 55.2\tiny$\pm$1.5 & 82.1\tiny$\pm$0.8 & 87.0\tiny$\pm$0.6 & 63.4\tiny$\pm$0.5 & \textbf{38.4}\tiny$\pm$2.2 & 81.4\tiny$\pm$0.9 & \textbf{75.5}\tiny$\pm$1.2 & 69.0 \\
\hline
QLoRA & 30b 8-bit & 55.8\tiny$\pm$1.5 & 82.5\tiny$\pm$0.8 & \textbf{87.4}\tiny$\pm$0.6 & \textbf{64.1}\tiny$\pm$0.5 & \textbf{38.8}\tiny$\pm$2.2 & \textbf{81.2}\tiny$\pm$0.9 & \textbf{75.4}\tiny$\pm$1.2 & \textbf{69.3} \\
Ours & 30b 8-bit & \textbf{56.1}\tiny$\pm$1.5 & \textbf{83.0}\tiny$\pm$0.8 & 86.8\tiny$\pm$0.6 & \textbf{64.1}\tiny$\pm$0.5 & 37.8\tiny$\pm$2.2 & \textbf{81.2}\tiny$\pm$0.9 & \textbf{75.4}\tiny$\pm$1.2 & 69.2 \\
\hline
\end{tabular}
\caption{Downstream task performance for LLaMA models fine-tuned on SlimOrca}
\end{subtable}
\caption{Performance of LLaMA models calibrated and fine-tuned on either Alpaca or SlimOrca with QuAILoRA or QLoRA on the validation splits of downstream tasks. In each comparison, the method that achieved higher accuracy is bolded; both are bolded if the difference in accuracy is less than 0.1\%. The confidence intervals presented are $\pm$ one standard error. Note that the standard errors for these results are greater than those for the training splits because the validation splits are much smaller. We observe the greatest positive advantage for the 7b parameter 4-bit quantized models, and mixed results for the larger and higher-bit quantized models.}
\label{table:downstream_tasks_validation}
\end{table*}

==> fig/mmlu_eval.tex <==
\begin{table*}[!t]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
FT Data & Model & Method & Acc. \\
\hline
 Alpaca & 7b 4-bit & QLoRA & \bf 31.4 \\
 Alpaca & 7b 4-bit & Ours & 30.2 \\
\hline
 Alpaca & 7b 8-bit & QLoRA & 31.0 \\
 Alpaca & 7b 8-bit & Ours & \bf 32.1 \\
\hline
 Alpaca & 13b 4-bit & QLoRA & 40.0 \\
 Alpaca & 13b 4-bit & Ours & \bf 41.5 \\
\hline
 Alpaca & 13b 8-bit & QLoRA & \bf 41.8 \\
 Alpaca & 13b 8-bit & Ours & 41.3 \\
\hline
 SlimOrca & 7b 4-bit & QLoRA & 30.7 \\
 SlimOrca & 7b 4-bit & Ours & \bf 32.2 \\
\hline
 SlimOrca & 7b 8-bit & QLoRA & \bf 30.5 \\
 SlimOrca & 7b 8-bit & Ours & 29.5 \\
\hline
 SlimOrca & 13b 4-bit & QLoRA & 42.8  \\
 SlimOrca & 13b 4-bit & Ours & \bf 45.0 \\
\hline
 SlimOrca & 13b 8-bit & QLoRA & 43.3 \\
 SlimOrca & 13b 8-bit & Ours & \bf 43.8  \\
\hline
\end{tabular}
\caption{Performance of LLaMA models fine-tuned on either Alpaca or Slim-Orca with QuAILoRA or QLoRA on MMLU. We do not observe any consistent advantage of one method over the other.}
\label{table:mmlu_eval}
\end{table*}

==> results.tex <==
\subsection{Perplexity after fine-tuning}

\input{fig/summarized_perplexity_table}

Here we compare the validation perplexity after fine-tuning 4-bit and 8-bit QLoRA models initialized with our method versus the baseline initialization.

The results are in Table \ref{table:summarized_perplexity_table}, and a breakdown of this 4-task average is in Appendix Table \ref{table:full_perplexity_table}. Results for the 8-bit OPT models are omitted due to errors encountered while fine-tuning these models using the BitsAndBytes and \verb|peft| libraries. We observe that in the vast majority of cases, fine-tuning a 4-bit or 8-bit QLoRA model using our initialization achieves lower validation perplexity than with the baseline initialization. In a small number of cases, the model initialized with our method achieves worse validation perplexity compared to the baseline initialization, which we present as failure cases. In some instances, the 4-bit model initialized with our method achieves even lower validation perplexity than the baseline 8-bit QLoRA model.

In the vast majority of cases, the 4-bit model initialized with our method outperforms the 4-bit QLoRA baseline and underperforms the 8-bit QLoRA baseline. This is expected behavior, since we do not expect our strategy for reducing quantization errors to be particularly bit-efficient. If the parameter quantization error $W-Q$ is rank-$r$, then indeed we can reduce quantization error to zero with our method by initializing $A$ and $B$ so that $AB^\top = W-Q$. However, we expect the parameter quantization errors $W-Q$ to instead be randomly distributed and far from low-rank, and therefore not easily reduced with our method.

We can use the results in Table \ref{table:summarized_perplexity_table} to compare the average reduction in validation perplexity that results from initializing a 4-bit QLoRA model with our method instead of the baseline initialization, versus the average reduction in validation perplexity that results from doubling the quantization precision from 4-bit to 8-bit precision when using the baseline initialization. To conduct this comparison, for each base model we compare the average validation perplexity across the four causal language modeling tasks for the 4-bit QLoRA baseline, 8-bit QLoRA baseline, and the 4-bit QLoRA model initialized with our method. We exclude LLaMa-30b from this average, since the 8-bit baseline model underperforms the 4-bit baseline on average. We also exclude the OPT-13b and OPT-30b LLMs, since we could not generate results for the 8-bit versions of these models. Averaging across LLaMa-13b, BLOOM-560m, BLOOM-3b, Pythia-70m, Pythia-410m, and Pythia-12b, the reduction in validation perplexity that results from initializing a 4-bit QLoRA model with our method is on average 75\% of that which results from doubling the quantization precision to 8-bit precision. The results of this analysis are in Table \ref{table:perplexity_gap_closed}.

We observe that in the LLaMA family of models, quantization error does not appear to significantly negatively affect validation perplexity after fine-tuning: the difference in validation perplexity after fine-tuning between the 4-bit and 8-bit baseline QLoRA models is small. Since our method improves performance by reducing quantization error, we observe that the gain in performance provided by our method over the baselines for the LLaMA models is proportionately small. For the other families, the difference in performance between the 4-bit and 8-bit baselines is significant enough for our method to provide a larger advantage over the baselines.

From these results, we conclude that initializing QLoRA with our method generally provides a moderate reduction in validation perplexity after fine-tuning, proportional to the negative affect of quantization error.

\subsection{Performance on downstream tasks}

%\input{fig/downstream_tasks}
\input{fig/downstream_tasks_train_split_summarized}

%%\input{latex/fig/downstream_tasks_slim-orca}
%%\input{latex/fig/mmlu_eval}

Here we compare how LLaMA models fine-tuned with QuAILoRA versus QLoRA on Alpaca or SlimOrca \citep{SlimOrca} perform on 7 downstream tasks: Arc-Challenge (Arc-C) \citep{allenai:arc}, Arc-Easy (Arc-E), BoolQ \citep{clark2019boolq}, HellaSwag (HS) \citep{zellers2019hellaswag}, OpenBookQA (OBQA) \citep{OpenBookQA2018}, PIQA \citep{Bisk2020}, and WinoGrande (WinoG) \citep{ai2:winogrande}. We use the EleutherAI LM Evaluation Harness \cite{eval-harness} for evaluation. For Alpaca experiments, we calibrate on Alpaca and fine-tune for one epoch. For SlimOrca experiments, we calibrate on SlimOrca and fine-tune on a random size-10000 subset of SlimOrca.  In order to accurately resolve the small difference in performance between QuAILoRA and QLoRA, we additionally evaluate on the training split of each task. Evaluating on the larger training splits yields more accurate evaluation metrics with tighter confidence intervals. The results for LLaMA 7b, 13b, and 30b parameter models on the validation splits of each task are in Table \ref{table:downstream_tasks_validation}, and the results for LLaMA 7b and 13b parameter models on the training splits are in Table \ref{table:downstream_tasks_train_split_thin}.

The confidence intervals we report in Tables \ref{table:downstream_tasks_validation} and \ref{table:downstream_tasks_train_split_thin} are the standard error. The formula for standard error is the sample standard deviation, divided by the square root of the number of evaluation samples. The standard error metrics that we report are produced directly by the EleutherAI evaluation harness \cite{eval-harness}.

Evaluating on the task validation splits, we observe a clear positive advantage for our method on the 7b parameter 4-bit quantized model, but inconclusive results for the other models. We observe that the difference in performance between the 4-bit and 8-bit quantized versions of the 13b and 30b parameter models is small. Therefore, we expect the observed gain in performance provided by our method over the baseline to be proportionately small. Indeed, the observed difference in performance is small compared to the computed confidence intervals, and so is statistically insignificant.

In order to better resolve the difference in performance between our method and the baseline, we additionally evaluate on the training splits of the evaluation tasks, which are typically much larger. We observe that the confidence intervals are much smaller when evaluating on the training splits. When evaluating on the training splits, we observe a much more statistically significant advantage for our method over the baseline on the 7b and 13b parameter 4-bit quantized models. Still, in many of the experiments using the 7b and 13b parameter 8-bit quantized models, the observed difference in performance between our method and the baseline is too small to be statistically significant.

%We observe much more mixed results between QuAILoRA and QLoRA on the validation splits than on the training splits: the difference in performance on each task between the two methods is much more likely to fall within a confidence interval of one standard error on the validation data. Still, the difference in performance is large enough to distinguish a positive advantage for our method over the QLoRA baseline on the 7b 4-bit quantized models, for which the negative impact on performance of quantization error is most significant.

%We observe a small, positive advantage for our method for the 7b and 13b parameter 4-bit quantized LLaMA models compared to the baseline. For the 8-bit quantized models, the advantage or difference in performance is small or statistically insignificant. For the 8-bit quantized models, this may be because the quantization error is already small, in which case reducing quantization error further with our method does not significantly improve performance. 

%The advantage of our method for the 13b parameter models appears to be smaller than for the 7b parameter models. This may be because the larger 13b parameter models are more robust to quantization error. This is supported by the observation that the difference in performance between the 4-bit and 8-bit 13b parameter models is much smaller compared to the difference in performance between the 4-bit and 8-bit 7b parameter models.


Averaged over all 7b and 13b parameter model experiments, the increase in accuracy observed on the validation splits for the 4-bit QuAILoRA model over the corresponding 4-bit QLoRA model is 43\% that of the increase in accuracy observed for the 8-bit QLoRA model over the corresponding 4-bit QLoRA model. For the training splits, the average increase is 65\%. We conclude that our method improves the downstream task performance of QLoRA on average, but that the affect may be insignificant when applied to models that are not significantly negatively affected by quantization error.

%%We support these results with further experiments in the appendix on the task validation splits, as well as experiments which show that our method provides a small positive advantage on validation perplexity after fine-tuning, especially for smaller and 4-bit quantized models where the affects of quantization errors are most significant.

%%\subsection{Time to quantize}

%%Here we compare to GPT-Q, a popular post-training quantization method. We observe that GPT-Q achieves higher performance, but that the computational overhead of our method is much smaller. It's possible that our method can be improved by combining with methods from the post-training quantization literature.

%\section{Downstream Validation Results}

%\input{fig/downstream_tasks}
%\input{latex/fig/downstream_tasks_slim-orca}
%\input{latex/fig/mmlu_eval}

%\section{MMLU Results}

%\input{fig/mmlu_eval}

%In addition to evaluating on the seven downstream tasks from the EleutherAI Evaluation Harness, we evaluate our fine-tuned 7b and 13b parameter LLaMA models on 5-shot MMLU. The results are in Table \ref{table:mmlu_eval}. Although we observe an increase in performance for our method in a majority of cases, the results are not sufficiently significant to be conclusive.

\subsection{Effect of LoRA rank}

\input{fig/lora_rank_fig}

%\input{latex/fig/lora_rank_table}

Here we examine the effect of the choice of the LoRA rank hyperparameter $r$ on performance after fine-tuning. We expect that using larger $r$ will allow our initialization of $A$ and $B$ to reduce a greater part of the quantization error and result in better performance after fine-tuning. A plot illustrating the effect of changing the LoRA rank when using our initialization versus the baseline initialization, averaged across six 4-bit LLMs (excluding Pythia-70m, LLaMa-30b and OPT-30b) and 4 causal language modeling tasks, is in Figure \ref{fig:lora_rank}. We observe that the performance of QLoRA generally increases as we increase the LoRA rank $r$, albeit with diminishing returns. In contrast, the choice of $r$ does not appear to significantly affect the performance of QLoRA when using the baseline initialization.

\subsection{Convergence of fine-tuning}

\input{fig/convergence_plot}

Here we examine how our method affects the speed of convergence of fine-tuning. In Figure \ref{fig:convergence_plots}, we plot the convergence curve for each of the fine-tuning experiments used to generate the validation perplexity results in Table \ref{table:finetune_table}. We plot fine-tuning steps on the horizontal axis and the average validation perplexity across the four causal language modeling tasks, measured every 100 fine-tuning steps, on the vertical axis. We observe that the 4-bit QLoRA models, when initialized with our method, achieve lower average validation perplexity at all stages of fine-tuning compared to the 4-bit QLoRA baselines. The difference in performance between the 8-bit QLoRA models fine-tuned with and without our method is on average much smaller compared to the 4-bit models, likely because the quantization error is already quite small for the 8-bit models and there are diminishing returns for reducing quantization error. From these plots, it appears that fine-tuning does not converge more quickly or slowly when initialized with our method compared to the baseline initialization. Rather, the benefit of decreased validation perplexity after fine-tuning observed for our method is due to decreased validation perplexity at initialization from decreased quantization error.

